LinearizeLLM: An Agent-Based Framework for LLM-Driven Exact Linear Reformulation of Nonlinear Optimization Problems

Reformulating nonlinear optimization problems into solver-ready linear optimization problems is often necessary for practical applications, but the process is often manual and requires domain expertise. We propose LinearizeLLM, an agent-based LLM framework that produces solver-ready linear reformulations of nonlinear optimization problems. Agents first detect the nonlinearity pattern (e.g., bilinear products) and apply nonlinearity pattern-aware reformulation techniques, selecting the most suitable linearization technique. We benchmark on 40 instances: 27 derived from ComplexOR by injecting exactly-linearizable operators, and 13 automatically generated instances with deeply nested nonlinearities. LinearizeLLM achieves 73\% mean end-to-end overall success (OSR) across nonlinearity depths (8.3x higher than a one-shot LLM baseline; 4.3x higher than Pyomo). The results suggest that a set of pattern-specialized agents can automate linearization, supporting natural-language-based modeling of nonlinear optimization.

==> depth_1_results.tex <==
% Auto-generated LaTeX fragment (no preamble).
% Source: data/results\_experiment\_1/Depth\_1
{\footnotesize
\subsection{problem\_blend\_problem\_abs}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\;
      &\; \sum_{j=1}^{J} p_j\,x_j
        \;+\;
        \sum_{i=1}^{I} \lambda_i\,
        \left|\;\sum_{j=1}^{J} c_{ij}\,x_j - d_i\right| \\[6pt]
\text{s.t.}\;
      &\; \sum_{j=1}^{J} x_j = 1 \\[4pt]
      &\; x_j \ge 0 \qquad && \forall\,j = 1,..,J
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $10.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $0.0$ \\
\texttt{z[0]} & $0.0$ \\
\texttt{z[1]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, z}\;
      &\; \sum_{j=1}^{J} p_j\,x_j
        \;+\;\sum_{i=1}^{I} \lambda_i\, z_i \\[6pt]
\text{s.t.}\;
      &\; \sum_{j=1}^{J} x_j = 1 \\[4pt]
      &\; x_j \ge 0 \qquad && \forall\,j = 1,..,J \\[4pt]
      &\; z_i \ge \sum_{j=1}^{J} c_{ij}\,x_j - d_i \qquad && \forall\,i = 1,..,I \\[4pt]
      &\; z_i \ge -\left(\sum_{j=1}^{J} c_{ij}\,x_j - d_i\right) \qquad && \forall\,i = 1,..,I \\[4pt]
      &\; z_i \ge 0 \qquad && \forall\,i = 1,..,I
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $10.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $0.0$ \\
\texttt{z[0]} & $0.0$ \\
\texttt{z[1]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_blend\_problem\_frac}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\;& 
    \frac{\sum_{i=1}^{3} c_i x_i}
         {\sum_{i=1}^{3} h_i x_i}
\\[8pt]
\text{s.t.}\;& 
    \sum_{i=1}^{3} h_i x_i \;\ge\; 7200
\\[10pt]
& \sum_{i=1}^{3} x_i \;=\; 1000
\\[4pt]
& x_i \;\ge\; 0\qquad (i=1,2,3).
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $0.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{t} & $0.0$ \\
\texttt{y[0]} & $0.0$ \\
\texttt{y[1]} & $0.0$ \\
\texttt{y[2]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{y,t}\;& 
    \sum_{i=1}^{3} c_i y_i
\\[8pt]
\text{s.t.}\;& 
    7200 t \;\le\; 1
\\[10pt]
& \sum_{i=1}^{3} y_i \;=\; 1000 t
\\[4pt]
& y_i \;\ge\; 0\qquad (i=1,2,3)
\\[4pt]
& t \;\ge\; 0.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $0.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{t} & $0.0$ \\
\texttt{y[0]} & $0.0$ \\
\texttt{y[1]} & $0.0$ \\
\texttt{y[2]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_diet\_problem\_min\_abs}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\quad &
      \Bigl|\;\sum_{j=1}^{J} p_j\,x_j \;-\; B\Bigr| \\[12pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} a_{ij}\,x_j \;\ge\;
      \min\!\Bigl(m_i,\;\sum_{j=1}^{J} a_{1j}\,x_j\Bigr)
      && \forall i = 1,\dots,I \\[6pt]
& \sum_{j=1}^{J} a_{ij}\,x_j \;\le\; M_i
      && \forall i = 1,\dots,I \\[6pt]
& \underline{x}_j \;\le\; x_j \;\le\; \overline{x}_j
      && \forall j = 1,\dots,J
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $9.333333333333334$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{b[0]} & $0.0$ \\
\texttt{b[1]} & $1.0$ \\
\texttt{x[0]} & $9.333333333333334$ \\
\texttt{x[1]} & $1.3333333333333333$ \\
\texttt{z\_abs\_1} & $9.333333333333334$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, z_{abs\_1}, b}\,\quad & z_{abs\_1} \\[12pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} p_j\,x_j \;-\; B \;\le\; z_{abs\_1} \\[6pt]
& B \;-\; \sum_{j=1}^{J} p_j\,x_j \;\le\; z_{abs\_1} \\[6pt]
& z_{abs\_1} \;\ge\; 0 \\[6pt]
& \sum_{j=1}^{J} a_{ij}\,x_j \;\ge\; m_i - M_i(1-b_i) && \forall i = 1,\dots,I \\[6pt]
& \sum_{j=1}^{J} a_{ij}\,x_j \;\ge\; \sum_{j=1}^{J} a_{1j}\,x_j - M_i b_i && \forall i = 1,\dots,I \\[6pt]
& b_i \;\in\; \{0,1\} && \forall i = 1,\dots,I \\[6pt]
& \sum_{j=1}^{J} a_{ij}\,x_j \;\le\; M_i
      && \forall i = 1,\dots,I \\[6pt]
& \underline{x}_j \;\le\; x_j \;\le\; \overline{x}_j
      && \forall j = 1,\dots,J
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $9.333333333333334$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{b[0]} & $0.0$ \\
\texttt{b[1]} & $1.0$ \\
\texttt{x[0]} & $9.333333333333334$ \\
\texttt{x[1]} & $1.3333333333333333$ \\
\texttt{z\_abs\_1} & $9.333333333333334$ \\
\hline
\end{tabular}\par}

\subsection{problem\_diet\_problem\_monotone}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\; & exp\left(\sum_{j=1}^{J} p_{j}\,x_{j}\right) \\[4pt]
\text{s.t.}\;
   & \underline{x}_{j} \;\le\; x_{j} \;\le\; \overline{x}_{j}
     && \forall\,j=1,\dots,J \\[6pt]
   & m_{i} \;\le\;
     \sum_{j=1}^{J} a_{i,j}\,x_{j}
     \;\le\; M_{i}
     && \forall\,i=1,\dots,I \\[6pt]
   & x_{j} \;\ge\; 0
     && \forall\,j=1,\dots,J
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $30740.40934396602$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{x[0]} & $4.666666666666667$ \\
\texttt{x[1]} & $0.6666666666666664$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x}\; & \sum_{j=1}^{J} p_{j}\,x_{j} \\[4pt]
\text{s.t.}\;
   & \underline{x}_{j} \;\le\; x_{j} \;\le\; \overline{x}_{j}
     && \forall\,j=1,\dots,J \\[6pt]
   & m_{i} \;\le\;
     \sum_{j=1}^{J} a_{i,j}\,x_{j}
     \;\le\; M_{i}
     && \forall\,i=1,\dots,I \\[6pt]
   & x_{j} \;\ge\; 0
     && \forall\,j=1,\dots,J
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $30740.40934396602$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{x[0]} & $4.666666666666667$ \\
\texttt{x[1]} & $0.6666666666666664$ \\
\hline
\end{tabular}\par}

\subsection{problem\_diet\_problem\_nonlinear\_frac}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\quad &
        \frac{\displaystyle\sum_{j=1}^{J} p_j\,x_j}
             {\displaystyle\sum_{j=1}^{J} x_j} \\[12pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} a_{ij}\,x_j \;\le\; M_i
      && \forall i = 1,...,I \\[6pt]
& \underline{x}_j \;\le\; x_j \;\le\; \overline{x}_j
      && \forall j = 1,..,J \\[6pt]
& \sum_{j=1}^{J} x_j \;\ge\; Q_{\min}
      && \text{(minimum total quantity)}
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $1.5$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{t} & $1.0$ \\
\texttt{y\_1} & $0.0$ \\
\texttt{y\_2} & $1.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{y,t}\quad & \displaystyle\sum_{j=1}^{J} p_j\,y_j \\[12pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} a_{ij}\,y_j - M_i\,t \;\le\; 0
      && \forall i = 1,...,I \\[6pt]
& \underline{x}_j\,t - y_j \;\le\; 0
      && \forall j = 1,..,J \\[6pt]
& y_j - \overline{x}_j\,t \;\le\; 0
      && \forall j = 1,..,J \\[6pt]
& \sum_{j=1}^{J} y_j - Q_{\min}\,t \;\ge\; 0
      && \text{(minimum total quantity, transformed)} \\[6pt]
& \sum_{j=1}^{J} y_j = 1
      && \text{(Charnes-Cooper transformation constraint)} \\[6pt]
& y_j \ge 0
      && \forall j = 1,..,J \\[6pt]
& t \ge 0
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $1.5$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{t} & $1.0$ \\
\texttt{y\_1} & $0.0$ \\
\texttt{y\_2} & $1.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_knapsack\_problem\_nonlinear\_min\_1}

\paragraph{Original model}

\[
\begin{aligned}
\max_{x}\quad & \sum_{j=1}^{J} v_j\,x_j \\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} w_j\,x_j - 10 \min \left\{x_1,\,x_3\right\}\;\le\; W, \\[6pt]
& x_j \;\in\; \{0,1\}
      \quad\forall j = 1,\dots,J.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $280.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $1.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\max_{x, \text{aux}_1}\quad & \sum_{j=1}^{J} v_j\,x_j \\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} w_j\,x_j - 10 \text{aux}_1 \;\le\; W, \\[6pt]
& \text{aux}_1 \;\le\; x_1, \\[6pt]
& \text{aux}_1 \;\le\; x_3, \\[6pt]
& x_j \;\in\; \{0,1\}
      \quad\forall j = 1,\dots,J, \\[6pt]
& \text{aux}_1 \;\in\; [0,1].
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $280.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $1.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_knapsack\_problem\_nonlinear\_min\_2}

\paragraph{Original model}

\[
\begin{aligned}
\max_{x}\quad & \sum_{j=1}^{J} v_j\,x_j + b \min \left\{x_1,\,x_2 \right\} \\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} w_j\,x_j \;\le\; W, \\[6pt]
& x_j \;\in\; \{0,1\}
      \quad\forall j = 1,\dots,J.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $220.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $0.0$ \\
\texttt{x[0]} & $-0.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $1.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\max_{x, \text{aux\_1}}\quad & \sum_{j=1}^{J} v_j\,x_j + b \cdot \text{aux\_1} \\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{J} w_j\,x_j \;\le\; W, \\[6pt]
& x_j \;\in\; \{0,1\}
      \quad\forall j = 1,\dots,J, \\[6pt]
& \text{aux\_1} \;\le\; x_1, \\[6pt]
& \text{aux\_1} \;\le\; x_2, \\[6pt]
& \text{aux\_1} \;\ge\; x_1 + x_2 - 1, \\[6pt]
& \text{aux\_1} \;\in\; \{0,1\}.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $220.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $0.0$ \\
\texttt{x[0]} & $-0.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $1.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_media\_selection\_nonlinear\_binbin}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\quad &
        \sum_{m=1}^{3} c_m\,x_m - d \cdot x_1 \cdot x_2 \\[6pt]
\text{s.t.}\quad
& \sum_{m=1}^{3} a_{t m}\,x_m \;\ge\; m_t
      && \forall t = 1,\dots,3, \\[6pt]
& x_m \;\in\; \{0,1\}
      && \forall m = 1,\dots,3.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $20.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, \text{aux\_1}}\quad &
        \sum_{m=1}^{3} c_m\,x_m - d \cdot \text{aux\_1} \\[6pt]
\text{s.t.}\quad
& \sum_{m=1}^{3} a_{t m}\,x_m \;\ge\; m_t
      && \forall t = 1,\dots,3, \\[6pt]
& \text{aux\_1} \;\le\; x_1 \\[6pt]
& \text{aux\_1} \;\le\; x_2 \\[6pt]
& \text{aux\_1} \;\ge\; x_1 + x_2 - 1 \\[6pt]
& x_m \;\in\; \{0,1\}
      && \forall m = 1,\dots,3, \\[6pt]
& \text{aux\_1} \;\in\; \{0,1\}.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $20.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_media\_selection\_nonlinear\_bincon}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x,q}\quad &
        \sum_{m=1}^{3} \left( c_m\,x_m - r_m x_m q_m\right)  \\[6pt]
\text{s.t.}\quad
& \sum_{m=1}^{3} a_{t m}\,x_m \;\ge\; m_t
      && \forall t = 1,\dots,3, \\[6pt]
& \sum_{m=1}^{3} q_m \leq 5 \\
& x_m \;\in\; \{0,1\}
      && \forall m = 1,\dots,3 \\
      & q_m \geq 0
      && \forall m = 1,\dots,3
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $15.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{q[0]} & $0.0$ \\
\texttt{q[1]} & $5.0$ \\
\texttt{q[2]} & $0.0$ \\
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $-0.0$ \\
\texttt{y[0]} & $0.0$ \\
\texttt{y[1]} & $5.0$ \\
\texttt{y[2]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x,q,y}\,\quad &
        \sum_{m=1}^{3} \left( c_m\,x_m - r_m y_m\right)  \\[6pt]
\text{s.t.}\quad
& \sum_{m=1}^{3} a_{t m}\,x_m \;\ge\; m_t
      && \forall t = 1,\dots,3, \\[6pt]
& \sum_{m=1}^{3} q_m \leq 5 \\
& y_m \leq q_m
      && \forall m = 1,\dots,3 \\
& y_m \leq 5 x_m
      && \forall m = 1,\dots,3 \\
& y_m \geq q_m - 5 (1 - x_m)
      && \forall m = 1,\dots,3 \\
& x_m \;\in\; \{0,1\}
      && \forall m = 1,\dots,3 \\
& q_m \geq 0
      && \forall m = 1,\dots,3 \\
& y_m \geq 0
      && \forall m = 1,\dots,3
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $15.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{q[0]} & $0.0$ \\
\texttt{q[1]} & $5.0$ \\
\texttt{q[2]} & $0.0$ \\
\texttt{x[0]} & $1.0$ \\
\texttt{x[1]} & $1.0$ \\
\texttt{x[2]} & $-0.0$ \\
\texttt{y[0]} & $0.0$ \\
\texttt{y[1]} & $5.0$ \\
\texttt{y[2]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_multi\_nonlinear\_abs}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\quad
& \sum_{i=1}^{2}\sum_{j=1}^{2}\sum_{p=1}^{2} c_{i,j,p}\,x_{i,j,p} + \sum_{j=1}^{2}\sum_{p=1}^{2} r \left|\sum_{i=1}^{2} x_{i,j,p} - \mathrm{Demand}_{j,p}\right| \\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2} x_{i,j,p} = \mathrm{Supply}_{i,p}
   && \forall\,i=1,2,\;\forall\,p=1,2,\\[4pt]
& \sum_{p=1}^{2} x_{i,j,p} \le \mathrm{Limit}_{i,j}
   && \forall\,i=1,2,\;\forall\,j=1,2,\\[4pt]
& x_{i,j,p} \ge 0
   && \forall\,i,j,p.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $240.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux[0,0]} & $0.0$ \\
\texttt{aux[0,1]} & $5.0$ \\
\texttt{aux[1,0]} & $0.0$ \\
\texttt{aux[1,1]} & $5.0$ \\
\texttt{x[0,0,0]} & $20.0$ \\
\texttt{x[0,0,1]} & $15.0$ \\
\texttt{x[0,1,0]} & $0.0$ \\
\texttt{x[0,1,1]} & $15.0$ \\
\texttt{x[1,0,0]} & $10.0$ \\
\texttt{x[1,0,1]} & $10.0$ \\
\texttt{x[1,1,0]} & $30.0$ \\
\texttt{x[1,1,1]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, \mathrm{aux}}
& \sum_{i=1}^{2}\sum_{j=1}^{2}\sum_{p=1}^{2} c_{i,j,p}\,x_{i,j,p} + \sum_{j=1}^{2}\sum_{p=1}^{2} r \, \mathrm{aux}_{j,p} \\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2} x_{i,j,p} = \mathrm{Supply}_{i,p}
   && \forall\,i=1,2,\;\forall\,p=1,2,\\[4pt]
& \sum_{p=1}^{2} x_{i,j,p} \le \mathrm{Limit}_{i,j}
   && \forall\,i=1,2,\;\forall\,j=1,2,\\[4pt]
& x_{i,j,p} \ge 0
   && \forall\,i,j,p.\\[4pt]
& \mathrm{aux}_{j,p} \ge \sum_{i=1}^{2} x_{i,j,p} - \mathrm{Demand}_{j,p}
   && \forall\,j=1,2,\;\forall\,p=1,2,\\[4pt]
& \mathrm{aux}_{j,p} \ge \mathrm{Demand}_{j,p} - \sum_{i=1}^{2} x_{i,j,p}
   && \forall\,j=1,2,\;\forall\,p=1,2,\\[4pt]
& \mathrm{aux}_{j,p} \ge 0
   && \forall\,j=1,2,\;\forall\,p=1,2.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $240.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux[0,0]} & $0.0$ \\
\texttt{aux[0,1]} & $5.0$ \\
\texttt{aux[1,0]} & $0.0$ \\
\texttt{aux[1,1]} & $5.0$ \\
\texttt{x[0,0,0]} & $20.0$ \\
\texttt{x[0,0,1]} & $15.0$ \\
\texttt{x[0,1,0]} & $0.0$ \\
\texttt{x[0,1,1]} & $15.0$ \\
\texttt{x[1,0,0]} & $10.0$ \\
\texttt{x[1,0,1]} & $10.0$ \\
\texttt{x[1,1,0]} & $30.0$ \\
\texttt{x[1,1,1]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_netasgn\_nonlinear\_abs}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\quad 
& \sum_{i=1}^{2}\sum_{j=1}^{2} c_{ij}\,x_{ij} + r\left|\sum_{j=1}^{2} x_{1j} - \sum_{j=1}^{2} x_{2j} \right|
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2} x_{ij} = S_i 
  && \forall\,i = 1,2, 
\\[4pt]
& \sum_{i=1}^{2} x_{ij} = D_j 
  && \forall\,j = 1,2, 
\\[4pt]
& 0 \;\le\; x_{ij} \;\le\; \ell_{ij} 
  && \forall\,i = 1,2,\; j = 1,2.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $297.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0,0]} & $2.0$ \\
\texttt{x[0,1]} & $6.0$ \\
\texttt{x[1,0]} & $3.0$ \\
\texttt{x[1,1]} & $4.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, aux_1}\quad 
& \sum_{i=1}^{2}\sum_{j=1}^{2} c_{ij}\,x_{ij} + r\,aux_1
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2} x_{ij} = S_i 
  && \forall\,i = 1,2, 
\\[4pt]
& \sum_{i=1}^{2} x_{ij} = D_j 
  && \forall\,j = 1,2, 
\\[4pt]
& 0 \;\le\; x_{ij} \;\le\; \ell_{ij} 
  && \forall\,i = 1,2,\; j = 1,2.
\\[4pt]
& \sum_{j=1}^{2} x_{1j} - \sum_{j=1}^{2} x_{2j} \le aux_1
\\[4pt]
& \sum_{j=1}^{2} x_{2j} - \sum_{j=1}^{2} x_{1j} \le aux_1
\\[4pt]
& aux_1 \ge 0
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $297.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0,0]} & $2.0$ \\
\texttt{x[0,1]} & $6.0$ \\
\texttt{x[1,0]} & $3.0$ \\
\texttt{x[1,1]} & $4.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_netasgn\_nonlinear\_max}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x}\quad 
& \sum_{i=1}^{2}\sum_{j=1}^{2} c_{ij}\,x_{ij} + r\max\left\{\left(\sum_{j=1}^{2} x_{1j} - \sum_{j=1}^{2} x_{2j}\right),\, \left(\sum_{j=1}^{2} x_{2j} - \sum_{j=1}^{2} x_{1j}\right)\right\}
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2} x_{ij} = S_i 
  && \forall\,i = 1,2, 
\\[4pt]
& \sum_{i=1}^{2} x_{ij} = D_j 
  && \forall\,j = 1,2, 
\\[4pt]
& 0 \;\le\; x_{ij} \;\le\; \ell_{ij} 
  && \forall\,i = 1,2,\; j = 1,2.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $297.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0,0]} & $2.0$ \\
\texttt{x[0,1]} & $6.0$ \\
\texttt{x[1,0]} & $3.0$ \\
\texttt{x[1,1]} & $4.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, aux_1}\quad 
& \sum_{i=1}^{2}\sum_{j=1}^{2} c_{ij}\,x_{ij} + r\,aux_1
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2} x_{ij} = S_i 
  && \forall\,i = 1,2, 
\\[4pt]
& \sum_{i=1}^{2} x_{ij} = D_j 
  && \forall\,j = 1,2, 
\\[4pt]
& 0 \;\le\; x_{ij} \;\le\; \ell_{ij} 
  && \forall\,i = 1,2,\; j = 1,2,
\\[4pt]
& aux_1 \ge \left(\sum_{j=1}^{2} x_{1j} - \sum_{j=1}^{2} x_{2j}\right)
\\[4pt]
& aux_1 \ge \left(\sum_{j=1}^{2} x_{2j} - \sum_{j=1}^{2} x_{1j}\right)
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $297.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $1.0$ \\
\texttt{x[0,0]} & $2.0$ \\
\texttt{x[0,1]} & $6.0$ \\
\texttt{x[1,0]} & $3.0$ \\
\texttt{x[1,1]} & $4.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_netmcol\_nonlinear\_bincon}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x, z}\quad & \sum_{(i,j)\in\mathcal{L}}\sum_{p\in\mathcal{P}} \left(ShipmentCost_{i,j,p} \cdot x_{i,j,p} - 0.2 \cdot ShipmentCost_{i,j,p} \cdot x_{i,j,p} \cdot z_{i,j}\right) + z_{i,j} \cdot ContractCosts_{i,j}\\
\text{s.t.}\quad
& \sum_{j:\,(j,i)\in\mathcal{L}} x_{j,i,p} + Supply_{i,p} = \sum_{j:\,(i,j)\in\mathcal{L}} x_{i,j,p} + Demand_{i,p}&& \forall i\in\mathcal{C},\;p\in\mathcal{P},\\
& x_{i,j,p} \;\leq\; Capacity_{i,j,p} && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P},\\
& \sum_{p\in\mathcal{P}} x_{i,j,p} \;\leq\; JointCapacity_{i,j} && \forall (i,j)\in\mathcal{L}, \\[6pt]
& x_{i,j,p} \;\geq\; 0 && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P} \\[6pt]
& z_{i,j} \;\in\; \left\{0,1\right\} && \forall (i,j)\in\mathcal{L}
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $10.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1[0,0,0]} & $0.0$ \\
\texttt{aux\_1[0,1,0]} & $0.0$ \\
\texttt{aux\_1[1,0,0]} & $0.0$ \\
\texttt{aux\_1[1,1,0]} & $0.0$ \\
\texttt{x[0,0,0]} & $0.0$ \\
\texttt{x[0,1,0]} & $10.0$ \\
\texttt{x[1,0,0]} & $0.0$ \\
\texttt{x[1,1,0]} & $0.0$ \\
\texttt{z[0,0]} & $0.0$ \\
\texttt{z[0,1]} & $0.0$ \\
\texttt{z[1,0]} & $0.0$ \\
\texttt{z[1,1]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, z, aux\_1}\quad & \sum_{(i,j)\in\mathcal{L}} \left( \sum_{p\in\mathcal{P}} \left(ShipmentCost_{i,j,p} \cdot x_{i,j,p} - 0.2 \cdot ShipmentCost_{i,j,p} \cdot aux\_1_{i,j,p}\right) + z_{i,j} \cdot ContractCosts_{i,j} \right)\\
\text{s.t.}\quad
& \sum_{j:\,(j,i)\in\mathcal{L}} x_{j,i,p} + Supply_{i,p} = \sum_{j:\,(i,j)\in\mathcal{L}} x_{i,j,p} + Demand_{i,p}&& \forall i\in\mathcal{C},\;p\in\mathcal{P},\\
& x_{i,j,p} \;\leq\; Capacity_{i,j,p} && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P},\\
& \sum_{p\in\mathcal{P}} x_{i,j,p} \;\leq\; JointCapacity_{i,j} && \forall (i,j)\in\mathcal{L}, \\[6pt]
& x_{i,j,p} \;\geq\; 0 && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P} \\[6pt]
& z_{i,j} \;\in\; \left\{0,1\right\} && \forall (i,j)\in\mathcal{L} \\[6pt]
% Added constraints for aux_1_{i,j,p} = x_{i,j,p} \cdot z_{i,j}
& aux\_1_{i,j,p} \;\leq\; Capacity_{i,j,p} \cdot z_{i,j} && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P} \\[6pt]
& aux\_1_{i,j,p} \;\leq\; x_{i,j,p} && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P} \\[6pt]
& aux\_1_{i,j,p} \;\geq\; x_{i,j,p} - Capacity_{i,j,p} \cdot (1 - z_{i,j}) && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P} \\[6pt]
& aux\_1_{i,j,p} \;\geq\; 0 && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P}
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $10.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1[0,0,0]} & $0.0$ \\
\texttt{aux\_1[0,1,0]} & $0.0$ \\
\texttt{aux\_1[1,0,0]} & $0.0$ \\
\texttt{aux\_1[1,1,0]} & $0.0$ \\
\texttt{x[0,0,0]} & $0.0$ \\
\texttt{x[0,1,0]} & $10.0$ \\
\texttt{x[1,0,0]} & $0.0$ \\
\texttt{x[1,1,0]} & $0.0$ \\
\texttt{z[0,0]} & $0.0$ \\
\texttt{z[0,1]} & $0.0$ \\
\texttt{z[1,0]} & $0.0$ \\
\texttt{z[1,1]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_netmcol\_nonlinear\_frac}

\paragraph{Original model}

\[
\begin{aligned}
\max_{x,y}\quad 
& \frac{\sum_{i\in\mathcal{C}}\sum_{p\in\mathcal{P}} r_p\,y_{i,p}}{
  \sum_{(i,j)\in\mathcal{L}}\sum_{p\in\mathcal{P}}
     ShipmentCost_{i,j,p}\,x_{i,j,p} + 0.01}
  \\[6pt]
\text{s.t.}\quad
& \sum_{j:\,(j,i)\in\mathcal{L}} x_{j,i,p}
  + Supply_{i,p}
  = \sum_{j:\,(i,j)\in\mathcal{L}} x_{i,j,p}
  + y_{i,p}
  && \forall i\in\mathcal{C},\;p\in\mathcal{P},
  \\[6pt]
& 0 \le y_{i,p} \le Demand_{i,p}
  && \forall i\in\mathcal{C},\;p\in\mathcal{P},
  \\[6pt]
& x_{i,j,p} \;\le\; Capacity_{i,j,p}
  && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P},
  \\[6pt]
& \sum_{p\in\mathcal{P}} x_{i,j,p}
  \;\le\; JointCapacity_{i,j}
  && \forall (i,j)\in\mathcal{L},
  \\[6pt]
& x_{i,j,p}  \;\ge\; 0
  && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P}.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $0.19980019980019983$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{t} & $0.09990009990009992$ \\
\texttt{x\_hat[0,0]} & $0.9990009990009991$ \\
\texttt{y\_hat[0,0]} & $0.0$ \\
\texttt{y\_hat[1,0]} & $0.9990009990009991$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\max_{\hat{x},\hat{y},t}\quad 
& \sum_{i\in\mathcal{C}}\sum_{p\in\mathcal{P}} r_p\,\hat{y}_{i,p}
  \\[6pt]
\text{s.t.}\quad
& \sum_{(i,j)\in\mathcal{L}}\sum_{p\in\mathcal{P}} ShipmentCost_{i,j,p}\,\hat{x}_{i,j,p} + 0.01\,t = 1
  \\[6pt]
& \sum_{j:\,(j,i)\in\mathcal{L}} \hat{x}_{j,i,p}
  + Supply_{i,p} \cdot t
  = \sum_{j:\,(i,j)\in\mathcal{L}} \hat{x}_{i,j,p}
  + \hat{y}_{i,p}
  && \forall i\in\mathcal{C},\;p\in\mathcal{P},
  \\[6pt]
& 0 \le \hat{y}_{i,p} \le Demand_{i,p} \cdot t
  && \forall i\in\mathcal{C},\;p\in\mathcal{P},
  \\[6pt]
& \hat{x}_{i,j,p} \;\le\; Capacity_{i,j,p} \cdot t
  && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P},
  \\[6pt]
& \sum_{p\in\mathcal{P}} \hat{x}_{i,j,p}
  \;\le\; JointCapacity_{i,j} \cdot t
  && \forall (i,j)\in\mathcal{L},
  \\[6pt]
& \hat{x}_{i,j,p}  \;\ge\; 0
  && \forall (i,j)\in\mathcal{L},\;p\in\mathcal{P},
  \\[6pt]
& t \ge 0
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $0.19980019980019983$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{t} & $0.09990009990009992$ \\
\texttt{x\_hat[0,0]} & $0.9990009990009991$ \\
\texttt{y\_hat[0,0]} & $0.0$ \\
\texttt{y\_hat[1,0]} & $0.9990009990009991$ \\
\hline
\end{tabular}\par}

\subsection{problem\_nltrans\_nonlinear\_bincon}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x, z}\quad & \left(1-z\right)\sum_{i=1}^{2}\sum_{j=1}^{2}r_{ij}\,x_{ij} + z\sum_{i=1}^{2}\sum_{j=1}^{2}\tilde{r}_{ij}\,x_{ij} + Cz
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2}x_{ij} \;\le\; S_i
      && \forall\,i = 1,2
\\[4pt]
& \sum_{i=1}^{2}x_{ij} \;\ge\; D_j
      && \forall\,j = 1,2
\\[4pt]
& 0 \le x_{ij} \;\le\; \ell_{ij}
      && \forall\,i,j = 1,2\\[4pt]
& z \in \left\{0,\,1\right\}
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $305.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux1} & $305.0$ \\
\texttt{aux2} & $0.0$ \\
\texttt{x[0,0]} & $5.0$ \\
\texttt{x[0,1]} & $15.0$ \\
\texttt{x[1,0]} & $25.0$ \\
\texttt{x[1,1]} & $5.0$ \\
\texttt{z} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x, z, \text{aux}_1, \text{aux}_2}\quad & \text{aux}_1 + \text{aux}_2 + Cz
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2}x_{ij} \;\le\; S_i
      && \forall\,i = 1,2
\\[4pt]
& \sum_{i=1}^{2}x_{ij} \;\ge\; D_j
      && \forall\,j = 1,2
\\[4pt]
& 0 \le x_{ij} \;\le\; \ell_{ij}
      && \forall\,i,j = 1,2\\[4pt]
& z \in \left\{0,\,1\right\}
\\[4pt]
& \text{aux}_1 \le 595 \left(1-z\right)
\\[4pt]
& \text{aux}_1 \ge 0
\\[4pt]
& \text{aux}_1 \le \sum_{i=1}^{2}\sum_{j=1}^{2}r_{ij}\,x_{ij}
\\[4pt]
& \text{aux}_1 \ge \sum_{i=1}^{2}\sum_{j=1}^{2}r_{ij}\,x_{ij} - 595z
\\[4pt]
& \text{aux}_2 \le \sum_{i=1}^{2}\sum_{j=1}^{2}\tilde{r}_{ij}\,x_{ij}
\\[4pt]
& \text{aux}_2 \ge \sum_{i=1}^{2}\sum_{j=1}^{2}\tilde{r}_{ij}\,x_{ij} - 465(1-z)
\\[4pt]
& \text{aux}_2 \le 465z
\\[4pt]
& \text{aux}_2 \ge 0
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $305.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux1} & $305.0$ \\
\texttt{aux2} & $0.0$ \\
\texttt{x[0,0]} & $5.0$ \\
\texttt{x[0,1]} & $15.0$ \\
\texttt{x[1,0]} & $25.0$ \\
\texttt{x[1,1]} & $5.0$ \\
\texttt{z} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_nltrans\_nonlinear\_max}

\paragraph{Original model}

\[
\begin{aligned}
\min_{x_{ij}\ge0}\quad & \sum_{i=1}^{2}\sum_{j=1}^{2}\left(r_{ij}\,x_{ij}+c\max\left\{0,\, x_{ij} - \ell_{ij} \right\} \right)
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2}x_{ij} \;\le\; S_i
      && \forall\,i = 1,2
\\[4pt]
& \sum_{i=1}^{2}x_{ij} \;\ge\; D_j
      && \forall\,j = 1,2
\\[4pt]
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $305.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{x[0,0]} & $5.0$ \\
\texttt{x[0,1]} & $15.0$ \\
\texttt{x[1,0]} & $25.0$ \\
\texttt{x[1,1]} & $5.0$ \\
\texttt{y[0,0]} & $0.0$ \\
\texttt{y[0,1]} & $0.0$ \\
\texttt{y[1,0]} & $0.0$ \\
\texttt{y[1,1]} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\min_{x_{ij}\ge0, y_{ij}\ge0}\quad & \sum_{i=1}^{2}\sum_{j=1}^{2}\left(r_{ij}\,x_{ij}+c\,y_{ij} \right)
\\[6pt]
\text{s.t.}\quad
& \sum_{j=1}^{2}x_{ij} \;\le\; S_i
      && \forall\,i = 1,2
\\[4pt]
& \sum_{i=1}^{2}x_{ij} \;\ge\; D_j
      && \forall\,j = 1,2
\\[4pt]
& y_{ij} \ge x_{ij} - \ell_{ij}
      && \forall\,i = 1,2,\,j = 1,2
\\[4pt]
& y_{ij} \ge 0
      && \forall\,i = 1,2,\,j = 1,2
\\[4pt]
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $305.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{x[0,0]} & $5.0$ \\
\texttt{x[0,1]} & $15.0$ \\
\texttt{x[1,0]} & $25.0$ \\
\texttt{x[1,1]} & $5.0$ \\
\texttt{y[0,0]} & $0.0$ \\
\texttt{y[0,1]} & $0.0$ \\
\texttt{y[1,0]} & $0.0$ \\
\texttt{y[1,1]} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_prod\_nonlinear\_bincon}

\paragraph{Original model}

\[
\begin{aligned}
\max_{x, z}\quad & \left(1 - z \right) \cdot \sum_{j=1}^{3} c_j \cdot x_j + z \cdot \sum_{j=1}^{3} \tilde{c}_j \cdot x_j - z \cdot C \\
\text{s.t.}\quad
& \sum_{j=1}^{3} \frac{1}{a_j} \cdot x_j \leq 4, \\
& 0 \leq x_j \leq u_j \quad \forall j = 1,2,3. \\[6pt]
& z \in \left\{0,\,1\right\}
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $55.66666666666667$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $55.66666666666667$ \\
\texttt{aux\_2} & $0.0$ \\
\texttt{x[0]} & $4.0$ \\
\texttt{x[1]} & $1.1666666666666667$ \\
\texttt{x[2]} & $3.0$ \\
\texttt{z} & $0.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\max_{x, z, aux_1, aux_2}\quad & aux_1 + aux_2 - z \cdot C \\
\text{s.t.}\quad
& \sum_{j=1}^{3} \frac{1}{a_j} \cdot x_j \leq 4, \\
& aux_1 \leq \sum_{j=1}^{3} c_j \cdot x_j, \\
& aux_1 \geq \sum_{j=1}^{3} c_j \cdot x_j - 104z, \\
& aux_1 \leq 104(1-z), \\
& aux_1 \geq 0, \\
& aux_2 \leq \sum_{j=1}^{3} \tilde{c}_j \cdot x_j, \\
& aux_2 \geq \sum_{j=1}^{3} \tilde{c}_j \cdot x_j - 125(1 - z), \\
& aux_2 \leq 125z, \\
& aux_2 \geq 0, \\
& 0 \leq x_j \leq u_j \quad \forall j = 1,2,3, \\
& z \in \left\{0,\,1\right\}
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $55.66666666666667$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $55.66666666666667$ \\
\texttt{aux\_2} & $0.0$ \\
\texttt{x[0]} & $4.0$ \\
\texttt{x[1]} & $1.1666666666666667$ \\
\texttt{x[2]} & $3.0$ \\
\texttt{z} & $0.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_prod\_nonlinear\_max}

\paragraph{Original model}

\[
\begin{aligned}
\max_{x}\quad & \sum_{j=1}^{3} c_j\,x_j - c\max\left\{0,\, \sum_{j=1}^{3} \frac{1}{a_j} \cdot x_j - b \right\}, \\[6pt]
\text{s.t.}\quad
& 0 \;\le\; x_j \;\le\; u_j
\quad \forall j = 1,2,3.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $89.5$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $4.833333333333333$ \\
\texttt{x[0]} & $4.0$ \\
\texttt{x[1]} & $6.0$ \\
\texttt{x[2]} & $3.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\max_{x, aux_1}\quad & \sum_{j=1}^{3} c_j\,x_j - c_{penalty}\,aux_1, \\[6pt]
\text{s.t.}\quad
& 0 \;\le\; x_j \;\le\; u_j
\quad \forall j = 1,2,3, \\[6pt]
& aux_1 \ge 0, \\[6pt]
& aux_1 \ge \sum_{j=1}^{3} \frac{1}{a_j} \cdot x_j - b.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $89.5$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $4.833333333333333$ \\
\texttt{x[0]} & $4.0$ \\
\texttt{x[1]} & $6.0$ \\
\texttt{x[2]} & $3.0$ \\
\hline
\end{tabular}\par}

\subsection{problem\_revenue\_maximization\_nonlinear\_bincon}

\paragraph{Original model}

\[
\begin{aligned}
\max_{x, z}\quad
& \left(1-z\right)\sum_{i=1}^{2} r_i\,x_i + z\sum_{i=1}^{2} \tilde{r}_i\,x_i - z \cdot C \\[6pt]
\text{s.t.}\quad
& \sum_{i=1}^{2} \delta_{ij}\,x_i \;\le\; c_j
      && \forall j = 1,2,3, \\[6pt]
& \underline{x}_i \;\le\; x_i \;\le\; \overline{x}_i
      && \forall i = 1,2, \\[6pt]
& x_i \in \mathbb{Z}
      && \forall i = 1,2, \\[6pt]
& z \in \left\{0,\, 1\right\} .
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $8000.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $0.0$ \\
\texttt{aux\_2} & $8800.0$ \\
\texttt{x[0]} & $20.0$ \\
\texttt{x[1]} & $40.0$ \\
\texttt{z} & $1.0$ \\
\hline
\end{tabular}\par}

\paragraph{Linearized model}

\[
\begin{aligned}
\max_{x, z, \text{aux\_1}, \text{aux\_2}}\quad
& \text{aux\_1} + \text{aux\_2} - z \cdot C \\[6pt]
\text{s.t.}\quad
& \sum_{i=1}^{2} \delta_{ij}\,x_i \;\le\; c_j
      && \forall j = 1,2,3, \\[6pt]
& \underline{x}_i \;\le\; x_i \;\le\; \overline{x}_i
      && \forall i = 1,2, \\[6pt]
& x_i \in \mathbb{Z}
      && \forall i = 1,2, \\[6pt]
& z \in \left\{0,\, 1\right\}, \\[6pt]
& \text{aux\_1} \le 9000 (1-z), \\[6pt]
& \text{aux\_1} \ge 0, \\[6pt]
& \text{aux\_1} \le \sum_{i=1}^{2} r_i\,x_i, \\[6pt]
& \text{aux\_1} \ge \sum_{i=1}^{2} r_i\,x_i - 9000 z, \\[6pt]
& 0 \le \text{aux\_1} \le 9000, \\[6pt]
% Added constraints for aux_2
& \text{aux\_2} \le 10000 z, \\[6pt]
& \text{aux\_2} \ge 0, \\[6pt]
& \text{aux\_2} \le \sum_{i=1}^{2} \tilde{r}_i\,x_i, \\[6pt]
& \text{aux\_2} \ge \sum_{i=1}^{2} \tilde{r}_i\,x_i - 10000 (1 - z), \\[6pt]
& 0 \le \text{aux\_2} \le 10000.
\end{aligned}
\]

{\centering
\begin{tabular}{@{}l r@{}}
\hline
\textbf{Objective} & $8000.0$ \\
\hline
\textbf{Variable} & \textbf{Value} \\
\hline
\texttt{aux\_1} & $0.0$ \\
\texttt{aux\_2} & $8800.0$ \\
\texttt{x[0]} & $20.0$ \\
\texttt{x[1]} & $40.0$ \\
\texttt{z} & $1.0$ \\
\hline
\end{tabular}\par}
}
